Counterfactual Explanations for Machine Learning: Challenges Revisited

Counterfactual explanations (CFEs) are an emerging technique under the umbrella of interpretability of machine learning (ML) models. They provide ``what if'' feedback of the form ``if an input datapoint were $x'$ instead of $x$, then an ML model's output would be $y'$ instead of $y$.'' Counterfactual explainability for ML models has yet to see widespread adoption in industry. In this short paper, we posit reasons for this slow uptake. Leveraging recent work outlining desirable properties of CFEs and our experience running the ML wing of a model monitoring startup, we identify outstanding obstacles hindering CFE deployment in industry.

==> reviews.tex <==
----------------------- REVIEW 1 ---------------------
SUBMISSION: 14
TITLE: Counterfactual Explanations for Machine Learning: Challenges Revisited
AUTHORS: Sahil Verma, John Dickerson and Keegan Hines

----------- Overall evaluation -----------
SCORE: 4 (Possibly accept: I would argue for accepting this paper)
----- TEXT:
The position paper first introduces the established concept of counterfactual explanations (CFEs) and their desired properties. Based on the authors' recent survey on that topic and their experience from the industry, they present a set of challenges for operationalizing CFEs. Therefore, the work fits well with the theme of the workshop. 

The position paper is well presented and follows a clear structure. 

Given that CFEs is a well-known and active research topic I am confident that the challenges presented could spark interesting discussions at the workshop. Therefore, I recommend acceptance.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 14
TITLE: Counterfactual Explanations for Machine Learning: Challenges Revisited
AUTHORS: Sahil Verma, John Dickerson and Keegan Hines

----------- Overall evaluation -----------
SCORE: 4 (Possibly accept: I would argue for accepting this paper)
----- TEXT:
Authors posit rationales behind the slow uptake of CFE and situate them in the context of a ML-based startup journey. They identify challenges around CFEs especially for industry deployment. The authors do a commendable job summarizing and situating their challenges. 

If the paper makes it to the final round of accepted work, the authors should address the following in the revised version:

- where applicable, bring in direct examples from their own experience to highlight the challenge

- comment on the feasibility of each of these challenges. Are these challenges ranked in terms of difficulty? 

- synthesize and conclude why and how these challenges (all taken together) has made CFE uptake difficult. This exercise is currently implied left to the reader and should be articulated from the authors. If space is an issue, consider cutting the image size and moving to the margins. 

I commend the authors for taking on this task and look forward to future iterations.



==> todos-camera-ready.tex <==
Review 1
Nothing

Review 2

1. Bring own examples to highlight challenges. 
2. Comment on the feasibility of each of these challenges. 
3. Synthesize and conclude why and how these challenges (all taken together) has made CFE uptake difficult. 


